Observations of compact sources in galaxy clusters using MUSTANG2

Compact sources can cause scatter in the scaling relationships between the amplitude of the thermal Sunyaev-Zel'dovich Effect (tSZE) in galaxy clusters and cluster mass. Estimates of the importance of this scatter vary - largely due to limited data on sources in clusters at the frequencies at which tSZE cluster surveys operate. In this paper we present 90 GHz compact source measurements from a sample of 30 clusters observed using the MUSTANG2 instrument on the Green Bank Telescope. We present simulations of how a source's flux density, spectral index, and angular separation from the cluster's center affect the measured tSZE in clusters detected by the Atacama Cosmology Telescope (ACT). By comparing the MUSTANG2 measurements with these simulations we calibrate an empirical relationship between 1.4 GHz flux densities from radio surveys and source contamination in ACT tSZE measurements. We find 3 per cent of the ACT clusters have more than a 20 per cent decrease in Compton-y but another 3 per cent have a 10 per cent increase in the Compton-y due to the matched filters used to find clusters. As sources affect the measured tSZE signal and hence the likelihood that a cluster will be detected, testing the level of source contamination in the tSZE signal using a tSZE selected catalog is inherently biased. We confirm this by comparing the ACT tSZE catalog with optically and X-ray selected cluster catalogs. There is a strong case for a large, high resolution survey of clusters to better characterize their source population.

==> Extra_plots.tex <==
\setcounter{page}{1}
\renewcommand{\thefigure}{4a}
\begin{figure*}
    \begin{center}
    \includegraphics[width=0.95\textwidth]{SED1.pdf}
    \end{center}
    \caption{ On-line Extra. SEDs for the sources found by MUSTANG2.  The MUSTANG2 flux densities assuming a point or an extended source at 10 arcsec resolution are shown by the green and yellow circles respectively -- not all sources show signs of extended emission in which case only the green point is visible. All points have error bars but many are too small to be easily seen.  The 1.4GHz data from FIRST/NVSS are in red, where available Herschel/SPIRE data is in blue, black points are from the VLA and BIMA, and the four high frequency points (in purple) are from WISE - note the lower two frequencies of these four points are mostly upper limits (all upper limits are shown as triangles).  The fitted spectral index between 90~GHz and 1.4~GHz is the red dashed line.  A 40~K black body spectrum with a 90~GHz flux density set at 20 per cent  of the measured MUSTANG2 flux density is shown in cyan.\newline
    Of the sources on this page, only those in MACS J0717.5+3745 have limits on the cold dust component. Those sources with counterparts (instead of upper limits) at 1.4~GHz all have spectral indices in the range expected from a synchrotron dominated source.}
     %The only counterpart to 01:05:34.2+13:23:07 came from the WISE data and there is a good chance this is a chance alignment -- With its upper limit at 1.4~GHz and inverted spectrum this source is likely to have a strong dust component.  Of other sources on this page 03:26:50.1-0043:40, 04:48:37.8-17:05:37, and 10:01:28.5+66:19:27 could have significant cold dust on top of a syncrotron component. A mixture of Herschel data and \comment{get reference for black point} in the cluster MACS J0717.5+3745 implies these two sources have very little dust but it is worth noting that 07:17:37.0+37:44:20 is slightly extended in both FIRST and MUSTANG data and the integrated flux density is likely brighter
  \end{figure*}    
  
\renewcommand{\thefigure}{4b}        
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{SED_zwicky.pdf}
    \caption{On-line Extra. SEDs for the sources found by MUSTANG2 in Zwicky 3146, with colors and symbols the same as the previous plot.  Zwicky 3146 had by far the most sources, enough that counterparts for some sources (e.g. 10:23:39.7+04:11:11 \& 10:23:38.7+04:11:05) are close enough to share the same Herschel counterpart.  Of the sources with a 28.5GHz counterpart, 10:23:45.3+04:10:43 \& 10:23:45.3+04:11:42, show a steepening of the spectral index towards 90~GHz. Steepening of source spectra at mm wavelengths is predicted by theory \citep{Kellermann1966,Blandford1979} and has been observed in many steep-spectra radio sources \citep[e.g.][]{Tucci2011}.  This feature is common in many other MUSTANG2 SEDs (e.g. 07:1737.0+37:44:20 and 13:47:30.6-11:45:10). In some cases this could be due to undetected extended 90~GHz emission around a strong core, however, for the analysis in this paper, this is a small source of error compared to uncertainties due to sample size and the assumption that the spectral index is the same in all sources. }% However 28.5GHz data is only available for a fraction of clusters so we the most useful spectral index for predicting source contamination is between 1.4~GHz and 90~GHz}
    
    %Zwicky 3146 has by far the most sources.  Herschel data limits the dust contribution in most cases with the exception 10:23:42.3+04:11:03 which may be dominated by dust.  More on this cluster can be found in \citet{Romero2020}. Few constrains on the type of emission at 90~GHz can be placed on the sources in MOO 1052+0823 or MOO 1054+0505. 
\end{figure*}    
\renewcommand{\thefigure}{4c}
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{SED2.pdf}
    \caption{On-line Extra. SEDs for the sources found by MUSTANG2 plotted with the same symbols and lines as previous SED plots. Of the sources in high-redshift MaDCoWS clusters (those with names beginning with MOO), 13:23:06.0-02:27:20 (and to some extent 11:11:14.1+68:38:49) show a highly inverted spectra with a 1.4~GHz counterpart that is an upper limit.  It is possible that a significant part of the 90~GHz flux from these sources is from cold dust.  The rest of the MaDCoWS clusters show more typical radio spectra yet at the same time have few constrains on a cold dust component.  In MACS~J1149.5+2223, Herschel data at 350 and 250~$\mu$m indicate the presence of cold dust but the upper limit at 500~$\mu$m shows that this emission is low at 90~GHz.  However, this could be an example of a source with a spectral index which is changing in the tSZE bands -- some dust could be present at frequencies above 150~GHz.  In RXJ~1347-1145 the Herschel data rules out any dust component at 90~GHz.  The measured flux of the point source is slightly lower than the 2016 measurements of \citet{Kitayama2016} which are in turn lower then the measurements from 2013 in \citet{Plagge2013}.  This could indicate long-term source variability.}
\end{figure*}    
\renewcommand{\thefigure}{4d}
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{SED3.pdf}
    \caption{On-line Extra. SEDs for the sources found by MUSTANG2 plotted with the same symbols and lines as previous SED plots. Again, sources in the MaDCoWS survey show the same pattern with very few constrains on a cold dust component and 1.4--90~GHz spectral indices consistent with radio emission -- with the exception of 15:53:59.1-04:47:50 which has only an upper limit at 1.4~GHz and an inverted spectra.  The Herschel data for the source in Abell~2052 shows this source is dominated by radio emission at 90~GHz yet at the same time the radio data are not well described by a single spectral index.  This could be due to a mixture of source variability, source geometry (faint extended emission not being included in the integrated fluxes) and real changes in the spectral index with frequency.}
\end{figure*}
